Incentives and Strategic Behaviour: An Experiment

How do incentive levels affect strategic behaviour? We address this with an experiment that separately identifies own- and opponent-incentive effects in two dominance-solvable games that differ in strategic complexity. Higher own incentives favour more strategically sophisticated actions and increase best responding to stated beliefs. Beliefs shift in a parallel direction and participants expect more sophisticated opponent actions. Furthermore, while higher own incentives increase belief accuracy, opponents with higher incentives are harder to predict. Higher incentives also increase response times, and longer response times are associated with better performance and more sophisticated actions and beliefs. Taken together, the evidence suggests that incentives affect strategic behaviour through two main channels: by reducing payoff-dependent mistakes and by increasing the effort devoted to reasoning, with the returns to that effort shaped by strategic complexity of the environment.

==> citepos.tex <==
% NATBIB CITEPOS COMMAND
\makeatletter
\DeclareRobustCommand\citepos													% Create possessives with \citepos[e.g.][p. Y]{Key}: e.g. Key's (Year, p. Y)
  {\begingroup\def\NAT@nmfmt##1{{\NAT@up##1's}}%
   \NAT@swafalse\let\NAT@ctype\z@\NAT@partrue
   \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}

\pretocmd{\NAT@citex}{%
  \let\NAT@hyper@\NAT@hyper@citex
  \def\NAT@postnote{#2}%
  \setcounter{NAT@total@cites}{0}%
  \setcounter{NAT@count@cites}{0}%
  \forcsvlist{\stepcounter{NAT@total@cites}\@gobble}{#3}}{}{}
\newcounter{NAT@total@cites}
\newcounter{NAT@count@cites}
\def\NAT@postnote{}


\def\NAT@hyper@citex#1{%														% Include postnote and \citet closing bracket in hyperlink
  \stepcounter{NAT@count@cites}%
  \hyper@natlinkstart{\@citeb\@extra@b@citeb}#1%
  \ifnumequal{\value{NAT@count@cites}}{\value{NAT@total@cites}}
    {\if*\NAT@postnote*\else\NAT@cmt\NAT@postnote\global\def\NAT@postnote{}\fi}{}%
  \ifNAT@swa\else\if\relax\NAT@date\relax
  \else\NAT@@close\global\let\NAT@nm\@empty\fi\fi								% Avoid compact citations
  \hyper@natlinkend}
\renewcommand\hyper@natlinkbreak[2]{#1}


\patchcmd{\NAT@citex}															% Avoid extraneous postnotes, closing brackets
  {\ifNAT@swa\else\if*#2*\else\NAT@cmt#2\fi
   \if\relax\NAT@date\relax\else\NAT@@close\fi\fi}{}{}{}
\patchcmd{\NAT@citex}
  {\if\relax\NAT@date\relax\NAT@def@citea\else\NAT@def@citea@close\fi}
  {\if\relax\NAT@date\relax\NAT@def@citea\else\NAT@def@citea@space\fi}{}{}
\patchcmd{\NAT@cite}{\if*#3*}{\if*\NAT@postnote*}{}{}
\makeatother
